Gaussian Belief Trees for Chance Constrained Asymptotically Optimal Motion Planning

In this paper, we address the problem of sampling-based motion planning under motion and measurement uncertainty with probabilistic guarantees. We generalize traditional sampling-based tree-based motion planning algorithms for deterministic systems and propose belief-$\mathcal{A}$, a framework that extends any kinodynamical tree-based planner to the belief space for linear (or linearizable) systems. We introduce appropriate sampling techniques and distance metrics for the belief space that preserve the probabilistic completeness and asymptotic optimality properties of the underlying planner. We demonstrate the efficacy of our approach for finding safe low-cost paths efficiently and asymptotically optimally in simulation, for both holonomic and non-holonomic systems.

==> sections/Algorithms.tex <==
\section{Algorithms}
\subsection{Sparse Stable RRBT with sampling bias}

The main algorithm we will consider is a variant of Sparse Stable RRT \cite{SST} for space 

==> sections/Analysis.tex <==
\section{Analysis}

\subsection{Completeness and Optimality}
\label{sec:convergence}
% Our sampling strategy completely samples the space of beliefs almost surely. With uniform sampling, the probability of expanding an existing node in the search space is proportional to the size of its Voronoi region. Heuristically biasing the growth towards lower uncertainty with a small probability improves the convergence rate 

% An important aspect of the Wasserstein metric is the preservation of the Lipschitz continuity of the state space's cost function to the Lipschitz continuity of the expected cost in the belief space \cite{importance}. For algorithms such as the Sparse Stable RRT, Lipschitz continuity is required for asymptotic near-optimality and probabilistic completeness.

The belief space extension inherits the probabilistic completeness and asymptotic (near)-optimality properties of the state space versions of the algorithms\footnote{A more thorough analysis can be found in the extended version of the paper \cite{ho2022arxiv}.}. The following theorems formalize these properties.

\begin{theorem}[Completeness]
    Algorithm belief-$\mathcal{A}$ is probabilistically complete for the stochastic system in \eqref{eq:system}
    if $\mathcal{A}$ is probabilistically complete for the nominal system in \eqref{eq:system} (without stochasticity).
\end{theorem}

% \begin{theorem}[Completeness]
%     If the underlying state space algorithm $\mathcal{A}$ is probabilistically complete under the nominal deterministic conditions (without stochasticity) in \eqref{eq:system}, algorithm belief-$\mathcal{A}$ is also probabilistically complete.
% \end{theorem}

% \ml{why is it important to have uniform sampling?}

\begin{proofsketch}
    Probabilistic completeness for tree-search algorithms requires that the search space is completely sampled almost surely.
    The main relevant consequence of the change to the belief space is the difference in sampling of the search space and propagation dynamics. However, with the sampling method described in~\ref{sec:sampling}, beliefs are sampled uniformly, which implies the search space is completely sampled almost surely (the inclusion of the bias term does not change the result). Additionally, if the dynamics is Lipschitz continuous, the propagation method presented in the belief space is also Lipschitz continuous. Hence, Belief-$\mathcal{A}$ inherits the probabilistic completeness properties of $\mathcal{A}$. 
\end{proofsketch}

The use of the 2-Wasserstein metric makes the new belief space a proper metric space, and it is known that the 2-Wasserstein metric preserves the Lipschitz continuity of the cost function~\cite{littlefield2018,kurniawati2013}. 
\begin{lemma}(Theorem in \cite{littlefield2018}).
    \label{lemma:lipschitz}
    For any control input $u \in \mathcal{U}$, if the cost function in the state space is Lipschitz continuous in the state space, then the expected cost function in the belief space with the 2-Wasserstein metric is also Lipschitz continuous.
\end{lemma}

\noindent Convergence guarantees for asymptotically ($\epsilon$-)optimal sampling-based planners typically rely on Lipschitz continuity in the cost function \cite{littlefield2018}.
This motivates the following theorem:

\begin{theorem}[Optimality]
    Belief-$\mathcal{A}$ is asymptotically ($\epsilon$-)optimal if algorithm $\mathcal{A}$ is asymptotically ($\epsilon$-)optimal under the conditions in Problem~\ref{env:problem}.
\end{theorem}
\begin{proofsketch}
    % If $\mathcal{A}$ is ($\epsilon-$)optimal, it implies that the cost function is Lipschitz continuous in the state and control space. 
    Since the cost function in Problem~\ref{env:problem} is Lipschitz continuous in the state and control space, by Lemma~\ref{lemma:lipschitz}, the cost function in the belief space under the 2-Wasserstein metric is also Lipschitz continuous. For belief-$\mathcal{A}$, the control space, method to sample controls and node selection procedure remains the same as $\mathcal{A}$. Hence, Belief-$\mathcal{A}$ inherits the asymptotic ($\epsilon$-)optimality properties of $\mathcal{A}$.
\end{proofsketch}
\subsection{Computational Efficiency}
The time complexity does not change for belief-$\mathcal{A}$ compared to $\mathcal{A}$, since the underlying tree-search algorithm remains the same. However, planning in the belief space increases computational effort in two ways. Firstly, planning in the belief space changes the dimension of the search space from $n$ state dimensions to $n + \frac{n(n-1)}{2}$ belief dimensions. Additionally, our extension changes subroutines to ones that are more computationally expensive than their state space analogues, specifically the distance metric for near/nearest neighbor queries and the Gaussian belief sampling method. Nevertheless, sampling-based algorithms scale reasonably well to higher dimensions, and the subroutines lead to fixed time increase per iteration. Empirically, as seen in the experiments, the belief space extension subroutines are reasonably efficient, allowing for fast planning in the belief space. We also compared to other approaches in the literature which solve similar problems in the belief space, in which our method is shown to have superior computational efficiency.

% For example, for a $2$ dimensional system if $\mathcal{A}$ is RRT with time complexity of $O( \mathtt{n}\log  \mathtt{n} +  \mathtt{n}\log^d  \mathtt{n})$, where $ \mathtt{n}$ is the number of tree nodes and $d = 2$ is the search space dimension, belief-$\mathcal{A}$ has the same time complexity but with $d = n + \frac{n(n-1)}{2} = 5$. Although this is more computationally expensive than usual state space planning, since n is fixed and does not grow with the number of iterations, this leads to a bounded computational time increase per iteration. 


% The use of the Wasserstein metric for nearest neighbor queries is slower than usual state space metrics. For general belief distributions, the Wasserstein metric has a time complexity of $O(N^3log N)$ for $N$ bin histograms. However, since our beliefs are Gaussian distributions, the Wasserstein distance computation in \eqref{eq:wasserstein} is more efficient, $O(n^3)$. This is higher than typical state space distance computations of $O(n)$. Similarly, we analyze the time complexity of sampling in this metric space. The time complexity of sampling random $n\times n$ matrix is $O(n)$, and that of QR decomposition is $O(n^3)$. Therefore, we have an overall time complexity for sampling of $O(n^3)$, which is higher than state space sampling of $O(n)$.

% \ml{use your RRT example here...  Therefore, the only change in the time complexity of belief-A compared to A is the increased dimensionality of the belief space... that is ... state d for belief space... then, use your RRT example... if A=RRT with time complexity of ..., then belief-RRT has the time compleixty of }

% Therefore, the main changes in the computation time of the belief-$\mathcal{A}$ compared to $\mathcal{A}$ is the increased dimensionality of the state space, and a fixed higher computational cost of the above subroutines per call. 

 

% \qh{Do we compare the time complexity of RRBT?}

% $\mathrm{n}, n, \mathsf{n}, \mathtt{n}$

==> sections/journalextensions.tex <==
1. Handling of noise when distribution is between multiple regions (maybe gaussian mixture?)
    1.a. Handle varying dynamics noise

2. Handling of nonlinear systems well
    2.a. EKF? - over-aprpoximate linearization error
    2.b. (Over-)approximations

3. Dynamic and unknown environments - better replanning strategy

4. More RRT algorithms

5. More concreteness of sampling bias (bias when needed)

5. Risk-awareness (Expectation, Var, CVaR)

5. Significantly more experiments
    a. Non-symmetric noise terms
    b. varying dynamics noise
    
6. Hardware demonstrations
